Approximating Cycles in Directed Graphs: Fast Algorithms for Girth and Roundtrip Spanners

The girth of a graph, i.e. the length of its shortest cycle, is a fundamental graph parameter. Unfortunately all known algorithms for computing, even approximately, the girth and girth-related structures in directed weighted $m$-edge and $n$-node graphs require $\Omega(\min\{n^{\omega}, mn\})$ time (for $2\leq\omega<2.373$). In this paper, we drastically improve these runtimes as follows: * Multiplicative Approximations in Nearly Linear Time: We give an algorithm that in $\widetilde{O}(m)$ time computes an $\widetilde{O}(1)$-multiplicative approximation of the girth as well as an $\widetilde{O}(1)$-multiplicative roundtrip spanner with $\widetilde{O}(n)$ edges with high probability (w.h.p). * Nearly Tight Additive Approximations: For unweighted graphs and any $\alpha \in (0,1)$ we give an algorithm that in $\widetilde{O}(mn^{1 - \alpha})$ time computes an $O(n^\alpha)$-additive approximation of the girth w.h.p, and partially derandomize it. We show that the runtime of our algorithm cannot be significantly improved without a breakthrough in combinatorial Boolean matrix multiplication. Our main technical contribution to achieve these results is the first nearly linear time algorithm for computing roundtrip covers, a directed graph decomposition concept key to previous roundtrip spanner constructions. Previously it was not known how to compute these significantly faster than $\Omega(\min\{n^\omega, mn\})$ time. Given the traditional difficulty in efficiently processing directed graphs, we hope our techniques may find further applications.

==> spanners_sequential.tex <==
\section{Round-trip Distance Spanners}
\label{sec:spanners}

\begin{figure}[ht]
	\noindent
	\centering
	\fbox{
		\begin{minipage}{6in}
            \noindent $(V_1, V_2, \ldots) = \textsc{Cluster-Out(-In)} (G, (v_1, \ldots, v_t), r_0, r)$, where $G = (V, E, l)$ is a directed graph, $v_1, \ldots v_t \in V$, $r_0 \geq 0$ and $r> 0$.
			\begin{enumerate}
                \item Set $\beta := \log n / (20\cdot r)$.
                \item Let $G_0 := G$.
                \item For $i$ in $1, \ldots, t$:
                    \begin{enumerate}
                        \item If $v_i$ is not in $G_{i-1}$, let $G_i := G_{i-1}, V_i := \emptyset$ and continue the loop. Otherwise:
                        \item Pick $x_i \sim \Exp(\beta)$.
                        \item Let $V_i := \outball_{G_{i-1}}(v_i, r_0 + x_i)$. ($\inball_{G_{i-1}}(v_i, r_0 + x_i)$ for $\textsc{Cluster-In}$)
                        \item Let $G_i := G_{i-1}$ with $V_i$ and incident edges removed.
                    \end{enumerate}
                \item Return $(V_1, V_2, \ldots, V_t, V \setminus \bigcup_i V_i)$, omitting empty sets.
			\end{enumerate}
		\end{minipage}
	}
	\caption{The clustering algorithm.}
	\label{fig:cluste-seq}
\end{figure}

\begin{figure}[ht]
	\noindent
	\centering
	\fbox{
		\begin{minipage}{6in}
            \noindent $(s^{out}, s^{in}) = \textsc{Estimate-Balls} (G, r, \epsilon)$, where $G = (V, E, l)$ is a directed graph and $r, \epsilon > 0$.
			\begin{enumerate}
                \item Sample $t = \lceil 20\cdot \log n / \epsilon^2 \rceil$ vertices $v_1, \ldots, v_t$  independently uniformly at random from $V$ with replacement.
                \item Compute the distances between every vertex in $V$ and each of $v_1, \ldots, v_t$.
                \item For each $u \in V$, let $s^{out}_u$ be the fraction of $v_1, \ldots, v_t$ such that $d_G(u, v_i) \leq r$.
                \item For each $u \in V$, let $s^{in}_u$ be the fraction of $v_1, \ldots, v_t$ such that $d_G(v_i, u) \leq r$.
                \item Return $(s^{out}, s^{in})$.
			\end{enumerate}
		\end{minipage}
	}
	\caption{The algorithm for estimating the sizes of out- and inballs at radius $r$ for a given graph.}
	\label{fig:estimate}
\end{figure}

\begin{figure}[ht]
	\noindent
	\centering
	\fbox{
		\begin{minipage}{6in}
            \noindent $\{C_1, C_2, \ldots\} = \textsc{Cover-Pass} (G, r)$, where $G = (V, E, l)$ is a directed graph and $r> 0$.
			\begin{enumerate}
                \item If $V$ is empty, return $()$.
                \item Let $s^{out}, s^{in} := \textsc{Estimate-Balls}(G, 400\cdot r, \frac{1}{8})$.
                \item Let $S^{out} := \{v \in V : s^{out}_v \geq \frac{3}{4}\}, S^{in} := \{v \in V : s^{in}_v \geq \frac{3}{4}\}$.
                \item If $S^{out} \cap S^{in} \neq \emptyset$:
                    \begin{enumerate}
                        \item Let $u \in S^{out} \cap S^{in}$.
                        \item Let $V^{out}, (V^{out})^* := \textsc{Cluster-Out}(G, (u), 400\cdot r, r)$ and $T^{out}$ be the corresponding tree from $u$.
                        \item Let $V^{in}, (V^{in})^* := \textsc{Cluster-In}(G, (u), 400\cdot r, r)$ and $T^{in}$ be the corresponding tree into $u$.
                        \item (\emph{failure}) If $|V^{out} \cap V^{in}| < \frac{1}{4} \cdot |V|$, return $V$ together with any in- and out-tree.
                        \item Let $C := (V^{out} \cap V^{in}, T^{out}, T^{in})$.
                        \item Let $G'$ be the graph induced by $G$ on $(V^{out})^* \cup (V^{in})^*$.
                        \item Return $\{C\} \cup \textsc{Cover-Pass}(G', r)$.
                    \end{enumerate}
                \item If $|S^{out}| \leq \frac{1}{2}\cdot|V|$:
                    \begin{enumerate}
                        \item Let $v_1, \ldots, v_{|V|}$ be any permutation of $V$ where vertices in $S^{out}$ come last.
                        \item Let $V_1, \ldots, V_t := \textsc{Cluster-Out}(G, (v_1, \ldots, v_{|V|}), 0, r)$.
                    \end{enumerate}
                 Otherwise (we have $|S^{in}| \leq \frac{1}{2}\cdot|V|$):
                    \begin{enumerate}
                        \item Let $v_1, \ldots, v_{|V|}$ be any permutation of $V$ where vertices of $S^{in}$ come last.
                        \item Let $V_1, \ldots, V_t := \textsc{Cluster-In}(G, (v_1, \ldots, v_{|V|}), 0, r)$.
                    \end{enumerate}
                \item (\emph{failure}) If $\max_i |V_i| > \frac{7}{8} \cdot |V|$, return $V$ together with any in- and out-tree.
                \item For $i = 1, \ldots, t$, let $G_i$ be the graph induced by $G$ on $V_i$.
                \item Return $\textsc{Cover-Pass}(G_1, r) \cup \ldots \cup \textsc{Cover-Pass}(G_t, r)$.
			\end{enumerate}
		\end{minipage}
	}
	\caption{Single pass of cover construction for a fixed radius.}
	\label{fig:pass}
\end{figure}

\begin{figure}[ht]
	\noindent
	\centering
	\fbox{
		\begin{minipage}{6in}
            \noindent $\{C_1, C_2, \ldots\} = \textsc{Fast-Roundtrip-Cover} (G, k, R)$, where $G = (V, E, l)$ is a directed graph and $k, R > 0$.
			\begin{enumerate}
                \item Let $r := R k \log n$.
                \item Let $\mathcal{C}_0 := \emptyset$.
                \item For $i = 1, \ldots, 20 \cdot \lceil n^{1/k} \rceil \cdot \lceil \log n \rceil$:
                \begin{align*}
                    \mathcal{C}_i := \mathcal{C}_{i - 1} \cup \textsc{Cover-Pass}(G, r).
                \end{align*}
                \item Return $\mathcal{C}$.
			\end{enumerate}
		\end{minipage}
	}
	\caption{The fast roundtrip cover algorithm.}
	\label{fig:cover}
\end{figure}

\begin{figure}[ht]
	\noindent
	\centering
	\fbox{
		\begin{minipage}{6in}
            \noindent $F = \textsc{Fast-Roundtrip-Spanner} (G, k)$, where $G = (V, E, l)$ is a directed graph and $k \geq 1$.
			\begin{enumerate}
                \item Let $(F_0, T) := \textsc{Roundtrip-$L_\infty$-Spanner}(G)$.
                \item For all $t \in \mathbb{Z}$, let $G^{(t)}$ be $G$ collapsed to $[2^t / n, 2^t \cdot n]$.
                \item Let $i := 0$.
                \item For every $t$ such that $G^{(t)}$ is nonempty:
                \begin{enumerate}
                    \item $F_{i + 1} := F_i \cup \mbox{ set of edges in } \textsc{Fast-Roundtrip-Cover}(G^{(t)}, k, 2^t)$.
                    \item $i := i + 1$.
                \end{enumerate}
                \item Return $F_i$.
			\end{enumerate}
		\end{minipage}
	}
	\caption{The roundtrip spanner algorithm.}
	\label{fig:spanner}
\end{figure}

\begin{figure}[ht]
	\noindent
	\centering
	\fbox{
		\begin{minipage}{6in}
            \noindent $s = \textsc{Find-Collapse-Time} (G, (e_L, \ldots, e_R))$, where $G = (V, E)$ is a directed graph, $L, R \in \mathbb{N}$ with $1 \leq L \leq R$.
			\begin{enumerate}
                \item If $L = R$, set $s_e = L$ for all $e \in E$ and return $s$.
                \item Let $M = \lfloor (L + R) / 2 \rfloor$.
                \item Let
                    \begin{align*}
                    E' := \{e \in E | e \mbox{ is contained inside a strongly connected component of the graph } (V, \{e_L, \ldots, e_M\})\}.
                    \end{align*}
                \item Let $V'$ be $V$ with edges in $E'$ contracted.
                \item Let $s' := \textsc{Find-Collapse-Time}((V, E'), (e_L, \ldots, e_M))$.
                \item Let $s'' := \textsc{Find-Collapse-Time}((V', E \setminus E'), (e_{M+1}, \ldots, e_R))$.
                \item Return $s'$ merged with $s''$.
			\end{enumerate}
		\end{minipage}
	}
	\caption{The recursive algorithm for computing collapse times.}
	\label{fig:collapse}
\end{figure}

\begin{definition}[\todo{RTZ}, modified]
    A collection $\mathcal{C}$ of triples $(V', T_{out}, T_{in})$ is a \emph{$(k,R)$-roundtrip-cover} of a directed graph $G = (V, E, l)$ if and only if each set $V'$ is of radius at most $k\cdot R$ as certified by trees $T_{out}$ and $T_{in}$, and for every pair of vertices $u, v \in V$ at roundtrip distance at most $R$, there exists a triple $(V', T_{out}, T_{in}) \in \mathcal{C}$ such that $u, v \in V'$.
\end{definition}

\begin{lemma}
\label{lem:cluster}
    Let $(V_1, V_2, \ldots)$ be the partition of $V$ returned by $\textsc{Cluster-Out}(G, (v_1, \ldots, v_t), r_0, r)$ (analogously of $\textsc{Cluster-In}$). Then:
    \begin{enumerate}
        \item the radii of the trees corresponding to all $V_i$ (except possibly the last one) are at most $r_0 + 400\cdot r$, whp., and
        \item for any pair of vertices $u, v$ at roundtrip distance at most $R$ in $G$, they are in the same set $V_i$ with probability at least
            \begin{align*}
                \exp(-\log n R / (20\cdot r)).
            \end{align*}
    \end{enumerate}
\end{lemma}
\Proof
Note that the maximum radius of any constructed tree is upper bounded by $r_0 + \max_i x_i$.
For every $i \in 1, \ldots, t$, we have
\begin{align*}
    Pr\left[x_i \geq 400 \cdot r\right] &\leq \exp(-400 \cdot \beta r)\\
                                        &= n^{-20},
\end{align*}
and so by union bound the maximum radius is at most $r_0 + 400 \cdot r$ with probability at least $1 - n^{-19}$.

To prove the
remainder of the lemma, fix two vertices $u$ and $v$ at roundtrip distance at most $R$ in $G$.
Assume the $i$-th cluster is the first one to contain an element of the set $\{u, v\}$.
By the memoryless property of the exponential distribution we see that conditioned on this event
the probability that cluster $i$ contains both vertices $u$ and $v$ is at least
\begin{align*}
    \Pr\left[\Exp(\beta)\geq R\right] = \exp(-\beta R),
\end{align*}
yielding the desired result.
\QED

\begin{lemma}
\label{lem:balls}
    Let $s^{out}, s^{in}$ be the output of $\textsc{Estimate-Balls}(G, r, \epsilon)$.
    For any vertex $u$, let $\bar{s}^{out}_u$ be the fraction of vertices in $V$ such that $d_G(u, v_i) \leq r$.
    Then, whp., for all vertices $u$ it holds that $|\bar{s}^{out} - s^{out}| \leq \epsilon$.
    An analogous statement holds for $s^{in}$.
\end{lemma}

\begin{lemma}
\label{lem:pass}
    Let $\mathcal{C} := \textsc{Cover-Pass}(G, r)$. Then:
    \begin{enumerate}
        \item for every $(V', T_{out}, T_{in}) \in \mathcal{C}$, the radii of $T_{out}$ and $T_{in}$ are $O(r)$, whp., and
        \item for any pair of vertices $u, v$ at roundtrip distance at most $R$ in $G$, they are in the same element of $\mathcal{C}$ with probability at least
            \begin{align*}
                \exp(-\log^2 n R / r),
            \end{align*}
        \item every vertex $v \in V$ belongs to exactly one element of $\mathcal{C}$, and
        \item the total size of the trees in $\mathcal{C}$ is $O(n)$.
    \end{enumerate}
\end{lemma}
\Proof
Properties 3. and 4. are easily verified.

To prove property 1., first note that whp. all calls to $\textsc{Cluster-In}, \textsc{Cluster-Out}$ and $\textsc{Estimate-Balls}$ yield the guarantees described in \Cref{lem:cluster,lem:balls}.
Conditioning on this event, we show that the failures in steps 4(d) and 6 of $\textsc{Cover-Pass}$ never occur; this is enough to show the thesis.
First assume that there exists a vertex $u \in S^{out} \cap S^{in}$.
Then, by assumption, we have $|\outball_G(u, 400\cdot r)| \geq \frac{5}{8}\cdot |V|$ and $|\inball_G(u, 400\cdot r)| \geq \frac{5}{8}\cdot |V|$.
Hence $|\outball_G(u, 400\cdot r) \cap \inball_G(u, 400\cdot r)| \geq \frac{1}{4} \cdot |V|$, which implies $|V^{out} \cap V^{in}| \geq \frac{1}{4}\cdot |V|$.
Hence the failure in step 4(d) cannot occur.
Now assume that $|S^{out}| \leq \frac{1}{2} \cdot |V|$ (the case $|S^{in}| \leq \frac{1}{2} \cdot |V|$ is analogous).
Since at least the first $\frac{1}{2} \cdot |V|$ of  $v_1, \ldots, v_{|V|}$ do not belong to $S^{out}$, and by assumption the radii of all balls grown in calls to $\textsc{Cluster-Out}$ are at most $400\cdot r$, the sizes of the clusters rooted at those vertices are of size at most $\frac{7}{8} \cdot |V|$ (by assumption on accuracy of $\textsc{Estimate-Balls}$).
The clusters assigned to the second half of $v_1, \ldots, v_{|V|}$ cannot be larger than $\frac{1}{2} \cdot |V|$ by construction.
Hence the failure in step 6 cannot occur.

To prove 2., first note that in every recursive call, the size of the vertex set is multiplied by at most $7/8$.
Therefore, there are at most $\lceil \log_{8/7} n \rceil$ levels of recursion.
Now fix two vertices $u$ and $v$ at roundtrip distance at most $R$ in $G$.
In each level of recursion, the vertex set is partitioned by at most two calls to $\textsc{Cluster-In}$ or $\textsc{Cluster-Out}$.
For each such partition, the probability $u$ and $v$ are not separated if they have not been separated previously is at least $\exp(-\log n R / (20\cdot r))$ by \Cref{lem:cluster}.
Hence, the probability that $u$ and $v$ are not separated at all is at least
\begin{align*}
    \exp(-\log n R / (20 \cdot r))^{\lceil \log_{8/7} n \rceil} &\geq \exp(-\log^2 n R / r).
\end{align*}
\QED

\begin{lemma}
    The collection $\mathcal{C}$ output by $\textsc{Fast-Roundtrip-Cover}(G, k, R)$ is an $(O(k \log n), R)$-roundtrip-cover of the directed graph $G = (V, E, l)$, w.h.p.
    Moreover, every vertex $v \in V$ belongs to $O(n^{1/k} \log n)$ elements of $\mathcal{C}$, and the total size of the trees in $\mathcal{C}$ is $O(n^{1 + 1/k} \log n)$.
\end{lemma}
\Proof
By \Cref{lem:pass}, whp. all trees in $\mathcal{C}$ are of radius $O(Rk \log n)$, and the size assertions are easily verified.

It remains to show that whp. any two vertices at short roundtrip distance share at least one cluster in $\mathcal{C}$.
Fix two vertices $u$ and $v$ at roundtrip distance at most $R$ in $G$.
By \Cref{lem:pass}, the probability they are in the same cluster in any single cover pass is at least $\exp(-\log^2 n R /r) = \exp(-\log n / k)$.
Hence, the probability they are separated in all of $\lceil n^{1/k} \rceil = \lceil \exp(\log n / k) \rceil$ independent passes is at most $\exp(-1)$.
Therefore, the probability they are separated in all the of $20 \cdot \lceil n^{1/k} \rceil \cdot \lceil \log n \rceil$ passes is at most $\exp(-20\log n) = n^{-20}$.
\QED

\begin{definition}
    Let $G = (V, E, l)$ be a directed graph and $x_L, x_R \in \mathbb{R}$ be such that $0 < x_L < x_R$.
    We construct $G$ \emph{collapsed} to $[x_L, x_R]$ by:
    \begin{itemize}
        \item merging any vertices that can reach each other while following only edges of length at most $x_L$,
        \item removing all edges longer than $x_R$,
        \item removing all edges whose endpoints cannot reach each other while following only edges of length at most $x_R$, and
        \item removing all vertices of degree $0$ remaining afer the above operations.
    \end{itemize}
\end{definition}

\begin{lemma}
    Let $G = (V, E, l)$ be a directed graph.
    For every $t \in \mathbb{Z}$, let $G^{(t)}$ be $G$ collapsed to $[2^t / n, 2^t \cdot n]$.
    Then the total number of edges in all $G^{(t)}$ is $O(m \log n)$, and the total number of vertices in all $G^{(t)}$ is $O(n \log n)$.
\end{lemma}

\begin{lemma}
    The output of $\textsc{Fast-Roundtrip-Spanner}(G, k)$ is an $O(k \log n)$-roundtrip-spanner of $G$ of size $O(n^{1+1/k} \log^2 n)$, whp.
\end{lemma}

